Evaluating Versal AI Engines for option price discovery in market risk analysis

Whilst Field-Programmable Gate Arrays (FPGAs) have been popular in accelerating high-frequency financial workload for many years, their application in quantitative finance, the utilisation of mathematical models to analyse financial markets and securities, is less mature. Nevertheless, recent work has demonstrated the benefits that FPGAs can deliver to quantitative workloads, and in this paper, we study whether the Versal ACAP and its AI Engines (AIEs) can also deliver improved performance. We focus specifically on the industry standard Strategic Technology Analysis Center's (STAC) derivatives risk analysis benchmark STAC-A2. Porting a purely FPGA-based accelerator STAC-A2 inspired market risk (SIMR) benchmark to the Versal ACAP device by combining Programmable Logic (PL) and AIEs, we explore the development approach and techniques, before comparing performance across PL and AIEs. Ultimately, we found that our AIE approach is slower than a highly optimised existing PL-only version due to limits on both the AIE and PL that we explore and describe.

==> notes_aie_dev_estimating_throughput.tex <==
\iffalse % comment starts

% https://docs.xilinx.com/r/en-US/ug1076-ai-engine-environment/Simulation-Input-and-Output-Data-Streams
From the output you can estimate the throughput of the designs for this PLIO port. Timestamps are related only to valid output. When the PLIO port is quiet, there is no indication on the output file. Compute the throughput as the number of output samples divided by the timestamp difference: $Throughput = NumberOfSamples / (LastTimestamp - FirstTimestamp)$. This simple equation will overestimate the throughput if you do not take into account all the clock cycles occuring after the last output sample. This might be highly overestimated if this is a frame-based output.\footnote{\url{https://docs.xilinx.com/r/en-US/ug1076-ai-engine-environment/Simulation-Input-and-Output-Data-Streams}}

example:
 
T 2168 ns
1.262882233e+00 
T 2172 ns
1.262882233e+00 
T 2176 ns
1.262882233e+00 
T 2180 ns
1.262882233e+00 
T 2184 ns
1.262882233e+00 
T 2188 ns
1.262882233e+00 
T 2192 ns
1.262882233e+00 
T 2196 ns
1.262882233e+00

throughput = 8 samples / (2196 ns - 2168 ns) 
throughput = 8 samples / 28 ns
throughput = 0.285714286 samples/ns
throughput = 2857.142857143 samples/ms
throughput = 2857142.857142857 samples/sec

% https://xilinx.github.io/Vitis-Tutorials/2021-1/build/html/docs/AI_Engine_Development/Design_Tutorials/07-firFilter_AIEvsHLS/README.html
It is important not to take that decision in isolation at the function level, but to look at the problem in relation to the complete dataflow path. For instance, an inefficient function implemented in the AI Engine may offer better total efficiency when preceded and followed in the dataflow by large amounts of efficient compute functions. It is likely that it will offer overall better throughput and latency than moving the data to the PL for that specific function and back into the AI Engine array.

For this discussion, computational efficiency is defined as the throughput (Msamples/sec) divided by power (W), and can only be used to compare designs that are identical from a functional standpoint. Given two identical designs with identical throughputs,for the purpose this tutorial, the one using less power is considered the better solution.

Window size

The AI Engine processes data in bursts and these data bursts are transferred between AI Engines utilizing ping-pong buffers. The data from one engine is written into one of the two buffers and when it is filled, the buffers are swapped and the data read out by the downstream engine. The size of these data bursts is referred to as the window size, and establishing the optimum window size is a balancing act between throughput and latency. Larger window sizes provide higher throughput because there the burst overhead is less of an influence on the performance. However, latency increases proportionately to the window size.

Thus, the window size should be chosen to be just large enough such that the desired throughput target is met.

% https://docs.xilinx.com/r/en-US/ug1504-acap-system-solution-planning-methodology/AI-Engine-Throughput-and-Latency

The data movement into, out of, and around the AI Engine array directly contributes to the latency of your system, for example, using window or streaming interfaces for your kernel. Depending on the window size, this can introduce an additional delay when loading the input, because the AI Engine waits for the full window to be available before starting the compute. With a streaming solution, the compute starts while the data is being delivered. Streaming interfaces are common for high data rate designs. However, this can lead to additional PL functionality being required to sort and align the data for streaming. In the case of the windowing solution, ping-pong buffering can help mitigate against the increased latency.

When communicating between the PL and AI Engine array, you must be aware of additional latency in your system if the PL is running more slowly than the AI Engine. In this case, you must use wider buses, (32, 64, or 128-bit) to bring the data into the array. This adds latency to the overall system, because the AXI4-Stream interconnect to the AI Engine memory and core is 32-bits, which adds 4 cycles to consume a 128-bit bus.

Tip: Use 64-bit PLIO at 500 MHz for best bandwidth utilization when feeding the AI Engine tiles in a -1 device where the AI Engine is running at 1 GHz.

%https://docs.xilinx.com/r/en-US/ug1076-ai-engine-environment/Event-Profile-APIs-for-Graph-Inputs-and-Outputs

\fi % comment ends

==> notes_aie_dev_kernel_descriptions.tex <==
\iffalse % comment starts

% notes:
\subsubsection{v01}
- naive scalar implementation\\
- only 32-bit wide streams\\
- single kernel\\
- ITERATIONS=500\\
\\
\subsubsection{v02}
- 4-way vectorised (single) kernel\\
- only 32-bit wide streams\\
- ITERATIONS=500/4=125 (as we compute four results per cycle)\\
\\
\subsubsection{v03}
- nine vectorised kernels\\
- 8-way\\
- using 256-bit windows between kernels\\
- 32-bit streams for scalar params\\
- 256-bit cascade stream for kernels which require three input params\\
- ITERATIONS=500/8=62.5=63 (as we compute eight results per cycle)\\
- (63\*8=504, hence last four results are obsolete)\\
\\
\subsubsection{v04}
- replicating loadV to have separate loads for s2 and m (reduce contention for same buffer from multicast)\\
- per 32-bit input stream to loadV/loadV\_duplicate, we read from input\_V.txt\\
- hence can read 64-bit per cycle per loadV kernel (128-bit per cycle for two loadV kernels)\\
\\
\\
\subsubsection{v05}
- providing two separate ports from input\_Z.txt for loadZ\\
- reduces the total cycles of load\_cascade\_fn from 10,774 to 10,763 (not very useful indeed.. sigh)\\

\subsubsection{v06}
- two parallel cascade streams along graph\\
- cascade stream: loadV     \-\> s2   \-\> psi  \-\> b2   \-\> b\\
- windows:                             /       \       \ \\
- cascade stream: loadV\_duplicate  \-\> m    \-\> a    \-\> v1qe\\
- windows:                                             / \\
-                                                      loadZ \\
\\
- parallel cascade streams connected with ping-pong buffer stall (lock stalls)\\
- so instead only have a single cascade stream\\
\\
- for single cascade stream along: loadV -$>$ s2 -$>$ psi -$>$ b2 -$>$ b\\
- and cascade along: loadV\_duplicate \-\> m\\
- and: a \-\> v1qe\\

\subsubsection{v07}
- like v06 but s2 \-\> psi and m \-\> psi both with windows (none with cascade stream)\\
- prevents cascade stream stalling between loadV and s2/m\\
- reduces s2\_fn total cycles from 3933 to 3332 (compared to v06)\\

\subsubsection{v20}
- same as v21\\
- but with 32-bit streams only and 4-way vectorisation\\

\subsubsection{v21}
- windows (no cascade) and 8-way vectorisation\\
- no separate load kernels, hence bottleneck is likely the 32-bit input for the 1st kernel in the graph\\
- variancePathQE / V1QE and logPricePathQE / Y1QE as two separate graphs\\
- both graphs not interconnected\\
- each kernel contains only a single 8-way vector operation (add\_fn, mul\_fn, negmul\_fn etc) opposite to previous versions where every kernel represents a function from the cpu code (m\_fn, s2\_fn, psi\_fn, a\_fn, b\_fn, v1qe\_fn)\\

\fi % comment ends

==> notes_table4_single_kernel_perf.tex <==
\begin{table*}[]
    \centering
    \caption{\textit{Single kernel} performance across PL and AIE: Total execution time in ms, averaged over five runs. AIE window size in bytes.} %\textcolor{red}{try in/out window 64 bytes, remaining inter-AIE windows flexible, so can use repackaging (repackage fails currently to generate working bitstream)}}
    \label{tab:single_kernel_perf}
    
    \begin{tabular}{c|c|cccc}
        \toprule
        \textbf{Description} & \makecell{\textbf{AIE}\\ \textbf{Window$<$size$>$}} & \textbf{Tiny} & \textbf{Small} & \textbf{Medium} & \textbf{Large} \\ 
        \midrule
        Alveo U280 \cite{stac-a2-h2rc} & - & 79.29 & 132.44 & 474.31 & 1370.13 \\ 
        %Streaming (H2RC 2022) VCK5000 PL - 1 CU & - & 146.62 & 275.03 & 696.14 & 2224.24 \\
        VCK5000 PL-only & - & 164.75 & 194.02 & 600.55 & 1718.93 \\
        \midrule
        naive scalar kernel & stream & 34366.74 & 68711.55 & 274903.37 & 819422.49 \\
        vectorised kernel & stream & 367.78 & 698.68 & 2709.01 & 8040.33 \\
    %    vectorised kernel & 32 & 406.94 & 788.98 & 3104.38 & 9197.58 \\
    %    vectorised kernel & 64 & 402.60 & 772.34 & 3008.08 & 8950.71 \\
        vectorised kernel & 128 & 361.22 & 690.15 & 2678.54 & 7961.03 \\
        multi-AIE & stream & 328.18 & 587.32 & 2309.43 & 6573.25 \\
    %    multi-AIE & 32 & 362.46 & 693.57 & 2693.21 & 8021.64 \\
        %VCK5000-nick & 64 & 354.90 & 688.28 & 2686.42 & 8035.17 \\ 
    %    multi-AIE & 64 & 323.25 & 580.77 & 1847.71 & 5346.56 \\ 
        %VCK5000-nick & 64 & 286.42 & 513.09 & 1776.90 & 5253.25 \\ 
        multi-AIE & 128 & 285.63 & 511.03 & 1531.56 & 4094.08 \\ 
        
        %multi-AIE \textcolor{red}{building} & 2048 & & & & \\ 
    %    one operation per kernel & 32 & &&& \\
    %    one operation per kernel & 64 & &&& \\
        one vector operation per kernel & 128 & 298.83 & 555.72 & 2153.28 & 6437.52 \\
        %\midrule
        %VCK5000-V3 & 32 & 597.33 & 1162.15 & 4546.88 & 13565.98 \\ 
        %VCK5000-V3 & 64 & 598.37 & 1161.42 & 4550.78 & 13560.55 \\ 
        %VCK5000-V3 & 2000 & 623.67 & 1217.13 & 4763.33 & 14209.61 \\ 
        %\midrule
        %VCK5000-V3-sendrecv-pipelined-II-51 & 32 & 2526.88 & 5020.06 & 19974.67 & 59820.95 \\ 
        \bottomrule
    \end{tabular}

\end{table*}

==> notes_table5_multi_kernel_perf.tex <==
\begin{table*}[]
    \centering
    \caption{\textbf{Multi kernel} performance across PL and AIE with total execution time in ms, averaged over five runs, AIE window size in bytes, \textit{stream} for AIE designs fully implemented with streams.}% \textcolor{red}{PL-only per CU, have 2 THREAD\_ON and 1 THREAD\_OFF} \textcolor{orange}{16.3 MB URAM limits CUs to 16 but 16 GB DRAM limits CUs to 10}}
    \label{tab:multi_kernel_perf}
    
    \begin{tabular}{c|c|cccc}
        \toprule
        \textbf{Description} & \makecell{\textbf{AIE} \\ \textbf{Window$<$size$>$}} & \textbf{Tiny} & \textbf{Small} & \textbf{Medium} & \textbf{Large} \\ 
        \midrule
        Alveo U280 - 6 CU \cite{stac-a2-h2rc} & - & 77.81 & 98.46 & 221.71 & 544.48 \\ 
        %VCK5000 PL-only - 4 CU & - & 178.53 & 199.14 & 286.88 & 649.51 \\
        %Streaming (H2RC 2022) VCK5000 PL - 6 CU & - & 182.54 & 338.39 & 897.54 & 1749.97 \\
        %Streaming (H2RC 2022) VCK5000 PL - 6 CU & - & &&& 597.99 \\
        %Streaming (H2RC 2022) VCK5000 PL - 8 CU \textcolor{red}{built} & - & & & & 231.11 \\
        VCK5000 PL-only - 10 CU & - & 170.11 & 266.38 & 412.16 & 932.76 \\
        \midrule
        %VCK5000 PL-only - 2 CU + 2 AIE subgraphs \textcolor{red}{building} & - & & & & \\
        multi-AIE - 6 CU \& 6 AIE subgraphs & stream & 336.88 & 521.17 & 1547.06 & 3198.02 \\
        %multi-AIE - 6 CU \& 6 AIE subgraphs & 32 & &&& \\ 
        %multi-AIE - 6 CU \& 6 AIE subgraphs & 64 & &&& \\ 
        multi-AIE - 6 CU \& 6 AIE subgraphs & 128 & 307.38 & 503.09 & 1543.63 & 3193.02 \\ 
        %one operation per kernel - 6 CU \& 6 AIE subgraphs & 32 & &&& \\ 
        %one operation per kernel - 6 CU \& 6 AIE subgraphs & 64 & &&& \\ 
        %one operation per kernel - 6 CU \& 6 AIE subgraphs & 128 & &&& \\ 
        \bottomrule
    \end{tabular}

\end{table*}

==> notes_table_aie_cycles.tex <==
\begin{table*}[]
    \centering
    \caption{Single kernel AIE performance in cycles. For more than one AIE kernel we report the earliest \textbf{Start} cycle and the latest \textbf{End} cycle of any kernel (\textbf{Total} cycles is the delta). We place one kernel per AIE, therefore the number of kernels matches the number of AIEs. There are 400 AIE available on the VCK5000. \textbf{Ver} for version, \textbf{Vec} for whether implemented as vector operation, \textbf{Comm} for data communication with \textbf{C} for cascade stream, \textbf{W} for windows, \textbf{S} for streams, \textbf{Util} for utilisation with \textbf{\# K} for number of kernels.}
    \label{tab:single_aie_kernel_cycles}
    
    %\resizebox{\textwidth}{!}{ % make table fit \textwidth
    \begin{tabular}{c|c|c|c|c|c|c|c|c} %|c|c}
    \toprule
    \multirow{2}{*}{\textbf{Description}} & \multirow{2}{*}{\textbf{Vectorisation}} & \multicolumn{3}{c|}{\textbf{Communication}} & \textbf{Utilisation} & \multicolumn{3}{c}{\textbf{Performance}} \\

    %\chline{4-11} % chline breaks the right border into two (because to rows), use cline instead
    %\cline{3-9}
    \cmidrule{3-9}
    
    & & {Cascade} & {Windows} & {Streams} &  {\# Kernels}  &  \makecell{Start\\cycle}  &  \makecell{End\\cycle}  &  \makecell{Total\\cycles}  \\ %&  \makecell{\%\\of v01} & \makecell{FLOP/\\cycle} \\ 
    
    \hline % \midrule % midrule looks worse than hline
    \makecell{naive scalar kernel}  & \xmark & \xmark & \xmark & \cmark & 1 & 615 & 642,207 & 641,592 \\ % & 100.00 & 0.02 \\ 
    \makecell{vectorised kernel}  & \cmark & \xmark & \xmark & \cmark & 1 & 615 & 19,222 & 18,607 \\ % & 2.90 & 5.20\\ 
    \makecell{vectorised kernel }  & \cmark & \cmark & \cmark & \cmark & 9 & 1,036 & 12,465 & 11,429 \\ % & 1.80 & 8.47\\ 
    \makecell{reading 128 bit per cycle for loadV}  & \cmark & \cmark & \cmark & \cmark & 10 & 1,080 & 11,977 & 10,897 \\ % & 1.70 & 8.88\\ 
    %\makecell{two separate ports from input\_Z for loadZ}  & \cmark & \cmark & \cmark & \cmark & 10 & 1,163 & 12,049 & 10,886 \\ % & 1.70 & 8.89\\ 
    %\makecell{two parallel cascade streams along graph}  & \cmark & $2\times$\cmark& \cmark & \xmark & 10 & 970 & 7,193 & 6,223 \\ % & 0.97 & 15.55\\ 
    %\makecell{loadv -$>$ s2/m with windows}  & \cmark & \cmark & \cmark & \xmark & 10 & 986 & 7,217 & 6,231 \\ % & 0.97 & 15.53\\ 
    %\makecell{one op/kernel (variancePathQE)}  & \cmark & \xmark & \cmark & \xmark & 34 & 2,453 & 30,747 & 28,294 \\ % & 4.40 & 3.42\\ 
    %\makecell{one op/kernel (variancePathQE + logPricePathQE}  & \cmark & \xmark & \cmark & \xmark & 45 & 3,034 & 30,302 & 27,268 \\ % & 4.30 & 3.55\\
    \bottomrule
    
    \end{tabular}%}
    
\end{table*}
